Lossy Quantum Source Coding with a Global Error Criterion based on a Posterior Reference Map

We consider the lossy quantum source coding problem where the task is to compress a given quantum source below its von Neumann entropy. Inspired by the duality connections between the rate-distortion and channel coding problems in the classical setting, we propose a new formulation for the lossy quantum source coding problem. This formulation differs from the existing quantum rate-distortion theory in two aspects. Firstly, we require that the reconstruction of the compressed quantum source fulfill a global error constraint as opposed to the sample-wise local error criterion used in the standard rate-distortion setting. Secondly, instead of a distortion observable, we employ the notion of a backward quantum channel, which we refer to as a "posterior reference map", to measure the reconstruction error. Using these, we characterize the asymptotic performance limit of the lossy quantum source coding problem in terms of single-letter coherent information of the given posterior reference map. We demonstrate a protocol to encode (at the specified rate) and decode, with the reconstruction satisfying the provided global error criterion, and therefore achieving the asymptotic performance limit. The protocol is constructed by decomposing coherent information as a difference of two Holevo information quantities, inspired from prior works in quantum communication problems. To further support the findings, we develop analogous formulations for the quantum-classical and classical variants and express the asymptotic performance limit in terms of single-letter mutual information quantities with respect to appropriately defined channels analogous to posterior reference maps. We also provide various examples for the three formulations, and shed light on their connection to the standard rate-distortion formulation wherever possible.

==> junk.tex <==
Future work:\\
- optimal distortion for QC.

In this work, we explored a new formulation of the source compression problem in the quantum, quantum-classical and classical settings.
The formulation is built on using  a global error criterion based on the notion of posterior channel that relates the source with the reconstruction. 
The posterior reference map is defined as a CPTP map, acting on the reference of the reconstruction to produce the reference of the source.
Using this formulation, we provide a single-letter characterizations of the asymptotic performance limits of the source coding problems in the three settings.
Furthermore, our work establishes the duality connection between the quantum source coding and chaneel coding problems. 


==> old_intro_Jan9th.tex <==
% \todo{1. Achievablity: Distinct codewords in Step 2.2 and 2.3}
% \todo{2. Converse: Complete the linear algebra lemma\\ Go through the converse.}
% \todo{3. Add pictures}
\todo{Introduction:\\ 1. Relevant work\\ 2. output statistics - Linder, aaron wagner, jun chen: optimal transport, weak coordination\\3. 
- global error (schumacher, goes to one as soon as rate is reduced below entropy)
- local error (in the classical setting, trades smoothly with distortion) \\4. add from proposal about duality }
\todo{define what transpose is?}
\todo{identification needed in packing lemma}
\todo{Subspace covering in terms of coherent information}
\todo{Classical paragraphs (cite normalized sandeep, weak coordination 2007 cuff).}

A fundamental problem from an information theoretic perspective is the asymptotic characterization of the rate required to compress a source that can be recovered to a certain measureable degree. Such a problem in quantum information theory is referred to as the quantum data compression problem.
In the lossless regime, Schumacher characterized this rate using the Von-Neumann entropy by providing a proof of achievability and the converse in the asymptotic setting. However, for the lossy regime, where the objective is to further reduce the rate at the expense of increased but bounded error, Barnum conjectured the minimum coherent information as the asymptotic limit. 

Generalizing the formulation from the classical rate-distortion theory \cite{Shannon}, Barnum introduced a distortion criterion as averaged single-letter entanglement fidelity (based on marginal operations) between the reconstruction and the original source. The minimization in the conjectured rate expression was then carried over all channels satisfying this distortion criterion. Supporting his conjecture, Barnum provided a lower bound to the rate-distortion function as coherent information, as well as a heuristical discussion of achievability. In this work, we revisit this problem and consider the task of characterizing a rate function, lower than Von-Neumann entropy, for compressing a purely quantum source while allowing for additional error in the reconstruction.  

In the literature on quantum information theory, a multitude of studies have relied on Barnum's rate distortion framework. The following are a few relevant works among many significant ones. 
1. Datta's QC rate distortion
2. Winters

From a duality standpoint, an interesting observation is that the channel coding problem, which is the dual of the source compression problem, has a well-characterized single-letter asymptotic performance limit. Precisely, this limit is obtained in terms of a single-letter coherent information between the reference and the output. Although many proofs followed ---, Devetak pioneered this result by employing a coherent approach to covering and packing results by combining them cohesively, inspired by his work on the private channel capacity problem.
This leads us to the question why is such a limit absent for the problem of lossy source compression?

An inherent problem lies with choosing a distortion criterion. While the averaged local-error distortion criteria renders itself adequately in classical formulations, including classical-quantum and quantum-classical setups, however, as we demonstrate in Section \ref{QLSC:sec:examples}, the letter-wise quantification of distortion breaks the essential entanglement (spread across the samples of the quantum source) needed for any meaningful reconstruction. As an example,
% we show in the sequel that even the dual of a fundamental hamming code, which perhaps appears to compress the quantum source without destroying its information, in the asymptotic limit renders a single-letter entanglement fidelity of 
% always pushes the single-letter distortion to its maximum value. 
we consider the task of compressing a quantum source using a dual of the commonly known hamming codes. We demonstrate through this example (Example \ref{example1}) that in the asymptotic limit, such codes behave poorly and approach a fidelity of half when measured using the single-letter entanglement fidelity criterion \nc. This motivates us to revisit the formulation of lossy compression even in the classical setting.

While looking at the classical setting, we find that in addition to Shannon's pioneering work of characterizing the rate distortion problem, there have been several works discussing the lossy source compression problem. Those that are of particular interest to us are the works of Verdu and ..., which have demonstrated that given a code that achieves the single-letter source compression limit of the rate distortion problem, that is, the mutual information between source and its reconstruction, also exhibits an interesting behaviour when it comes to the so called the reverse test channel. In particular, the reverse test channel resulting from such codes behaves like a  product channel, with 1 revealing the closeness in normalized divergence and 2 in total variation.

In light of this, in this work, we embark on a journey to explore a different formulation of the source compression problem. More precisely, we want to design an encoder and decoder such that the joint effect of encoding and decoding is close to the effect of a given product reverse channel acting on a non-product reconstruction. Although we have a clear notion of a reverse test channel classically, such a channel is not uniquely defined in a purely quantum setting. Petz recovery map is one such channel which has found quite relevance in information theoretic problems. However, we digress here and consider a new map acting on the reference of the reconstruction with an existence, as we show in the sequel, guaranteed using the famous Uhlmann's theorem. 

% The contributions of our work can be summarized as follows
Using this new map, we provide a new formulation to the quantum lossy source coding problem. 
 Considering such formulation, we ask the question, is it possible to obtain a single letter characterization of the performance asymptotic performance limit to the considered problem formulation? As a main contribution of our work we show that the coherent information of the posterior reference map $W$ forms the single letter performance limit of the source coding problem. 
 Moreover, our work also provides an answer to the missing duality between the quantum lossy compression and quantum channel coding problems.
Furthermore, as will become evident, the proof relies on the coherent application of the two fundamental tools of quantum information theory, packing and covering, suggesting a connection with the proof of Devetak for the channel coding problem. Nonetheless, the application here is more involved, as is common for any source coding problem. For instance, the coherent covering used requires additional rotation unitary operations to ensure a larger subsystem is covered. Similarly, coherent packing borrowed ideas from quanutm communication with side information to release redundant correlated information into the environment without destroying the entanglement.

 % However, one may wonder as to what would happen when the above coherent information is negative, 
 However, unlike quantum mutual information (which forms the asymptotic limit in the setting of entanglement assistance) coherent information can at times be negative, while rate required to compress is always non-negative. Investigating this discord/incompatibility/conflict, we  realized that in such cases, when posterior reference map is such that coherent information becomes negative, no amount of quantum resources are needed to provide a satisfactory reconstruction.
 % that satisfies the proposed error criterion (\eqref{def:protocolError}). 
 A cheaper resource, such as classical storage, local randomness, and local unitary evolutions are sufficient to achieve the task. In this regard, for such situation, we reformulate the problem as compressing the classical outcomes while maintaining the association with the reference. In particular, in Section \nr we formulate the problem as a measurement compression problem \cite{winter} except that it only requires the \emph{faithful simulation} of the reference system. 

 Finally, to further corroborate the findings, we also provide a converse to the asymptotic performance limit of the formulated problem in terms of single-letter quantities. For the fully quantum compression problem, we show that the rate cannot be lower than the single-letter coherent information with respect to the given isometric map $W$. Similarly, in the quantum-classical and purely classical setting, we achieve a lower bound of respective mutual information quantities with respect to the posterior map and distribution, respectively. The tight converses implies the tightness of the achievable inner bounds.


==> old_proofs.tex <==

\error{\subsection{Old - Proof of Proposition \ref{prop:ExpectedFourier}}}
Observe that using \eqref{eq:Ma_orthogonal}, we have the collection $\{|{\chi_{k}^{(m)}}\rangle\}_{k\in\calK}$ as an orthonormal collection of states for all $m\in \calM$.  Similarly, using the orthogonality of $\Pi_k^{(m)}$ and the condition $\IndDC=1$, the collection $\{|{\phi_{k}^{(m)}}\}_{k\in\calK}$ is orthonormal for all $m\in \calM$. 
Define the Fourier transform states corresponding to the collections $\curlys{\chi_k^{(m)}}$ and  $\curlys{\phi_k^{(m)}}$ as
\begin{align}
    |{\hat{\chi}_s^{(m)}}\rangle \deq \frac{1}{\sqrt{|\calK|}}\sum_{k}e^{\frac{2\pi i ks}{|\calK|}}|{\chi_k^{(m)}}\rangle \qand     |{\hat{\phi}_s^{(m)}}\rangle \deq \frac{1}{\sqrt{|\calK|}}\sum_{k}e^{\frac{2\pi i ks}{|\calK|}}|{\phi_k^{(m)}}\rangle. \nonumber
\end{align}
It follows from Parseval's Theorem,
\begin{align}
    \frac{1}{|\calK|}\sum_{s\in \calK} \langle{\hat{\phi}_s^{(m)}}|{\hat{\chi}_s^{(m)}}\rangle = \frac{1}{|\calK|}\sum_{ k\in \calK} \langle{{\phi}_k^{(m)}}|{{\chi}_k^{(m)}}\rangle. \nonumber
\end{align}
Taking expectation over the codebook generation, and using \eqref{eq:avg_packing_error} gives,
\begin{align}
   \frac{1}{|\calK|}\sum_{s \in \calK} \EE\left[ \langle{\hat{\phi}_s^{(m)}}|{\hat{\chi}_s^{(m)}}\rangle\right] = \frac{1}{|\calK|}\sum_{k \in \calK} \EE\left[\langle{{\phi}_k^{(m)}}|{{\chi}_k^{(m)}}\rangle\right] \geq 1-\epsilon \mbox{ for all } m\in \calM. \nonumber
\end{align}
Therefore, for all $m\in \calM$, there exists at least one value of $s_m \in \calK$ that follows the inequality: $$e^{i\hat\theta_m} \EE\left[ \langle{\hat{\phi}_{s_m}^{(m)}}|{\hat{\chi}_{s_m}^{(m)}}\rangle\right] \geq 1-\epsilon, \quad \mbox{for some phase } \hat{\theta}_m. $$
Choosing $\alpha_k^{(m)} = \frac{2\pi k s_m}{|\calK|}$ and $\beta_k^{(m)} = \frac{2 \pi k s_m}{|\calK|} - \hat\theta_m$, we obtain
\begin{align}
    \frac{1}{|\calM|}\sum_{m}\EE\left[ \langle\phi_m|\chi_m\rangle \right] \geq 1-\epsilon.
\end{align}
% Once we have chosen the phases $\alpha_k^{(m)}$ and $\beta_k^{(m)}$, choose the phase $\theta_\calC$ such that $$e^{i\theta_\calC}\sum_{m\in\calM}\langle\phi_m|\chi_m\rangle = |\sum_{m\in\calM}\langle\phi_m|\chi_m\rangle|.$$ 
This means that 
\[
 \frac{1}{|\calM|}\sum_{m}\EE\left[ \mbox{Re}\langle\phi_m|\chi_m\rangle \right] \geq 1-\epsilon,
\]
and consequently,
\begin{align}
     \frac{1}{|\calM|}\EE\left|\sum_{m} \langle\phi_m|\chi_m\rangle \right| \geq \frac{1}{|\calM|}\EE\bigg[\mbox{Re}\left( \sum_{m}\langle\phi_m|\chi_m\rangle\right) \bigg] = \frac{1}{|\calM|}\sum_{m}\EE\bigg[\mbox{Re}\left( \langle\phi_m|\chi_m\rangle \right)\bigg] \geq 1-\epsilon.
\end{align}
This completes the proof.





\section{Old proof of Outer Bound}

\begin{align}
    nR \geq S(A^n)_{\omega} = S(E^n \bBn)_{\omega} = S(\bBn)_{\omega} + S(E^n |\bBn)_{\omega}  \geq S(\bBn)_{\omega} - S(E^n)_{\omega} = S(\bBn)_{\omega} - S(A^n\!,\bBn)_{\omega}, \nonumber
\end{align}
where $\calH_{E^n}$ is assumed to purify the state $\omega^{\bB^n A^n}$, and the last inequality uses the strong subadditivity of conditional mutual information \cite[Theorem 10.6.1]{wilde_arxivBook} as
\begin{align}
    0 & \leq I(E^n, A^n | \bBn)_{\omega} = S(E^n|\bBn)_{\omega} - S(E^n|\bBn, A^n)_{\omega} \nonumber \\
    &  = S(E^n|\bBn)_{\omega} - S(E^n,\bBn, A^n)_{\omega} - S(\bBn, A^n)_{\omega}     = S(E^n|\bBn)_{\omega}  - S(E^n)_{\omega}. 
\end{align}
Using the fact that $S(\bBn)_\omega = nS(\bB)_\omega$, and the result conditioning reduces entropy \cite[Theorem 11.4.1]{wilde_arxivBook}, we obtain
\begin{align}
    nR \geq nS(\bB)_{\omega} - \sum_{i=1}^{n} S(\bB_i, A_i)_{\omega}.
\end{align}
Define the states $\tau^{\bBQ \AQ}, \mu^{\bBQ \AQ} \in \calD(\calH_{\bB}\tensor \calH_{\bA})$ as
\begin{align}
    \tau^{\bBQ \AQ} &\deq \frac{1}{n}\sum_{i=1}^n \Tr_{\Ani \bBni}\{\omega^{\bBn A^n}\} \qand \nonumber \\
    \mu^{\bBQ \AQ} &\deq (\bV\tensor I)\bigg(\frac{1}{n}\sum_{i=1}^n \Tr_{\Ani \bAni}\{\Psi^{\bAn A^n}_{\omega}\}\bigg)(\bV\tensor I)^{\dagger}.
\end{align}
From the concavity of entropy, we know $\sum_{i=1}^{n} S(\bB_i, A_i)_{\omega} \geq nS(\bBQ \AQ)_{\tau}$, which gives
\begin{align}
    nR \geq nS(\bB)_{\tau} - nS(\bBQ \AQ)_{\tau}.
\end{align}
Now consider, 
\begin{align}
    \| \tau^{\bBQ \AQ}  - \mu^{\bBQ \AQ}\|_1 & \leq \frac{1}{n}\sum_{i=1}^n \left\| \Tr_{\Ani \bBni}\{\omega^{\bBn A^n}\} - (\bV\tensor I)\bigg(\frac{1}{n}  \Tr_{\Ani \bAni}\{\Psi^{\bAn A^n}_{\omega}\}\bigg)(\bV\tensor I)^{\dagger} \right\| \nonumber \\
    & \leq \frac{1}{n}\sum_{i=1}^n \left\|  \omega^{\bBn A^n}  - \upsilon^{\bBn A^n}\right\| \leq \epsilon
\end{align}
where the first inequality follows from triangle inequality, the second uses the fact that  $V^\dagger V = I$ and the monotonicity of trace distance, and the last follows from \eqref{eq:cons_conv1}

==> quantum_header_2.tex <==
%========================================================================================
%------------------------- This header contains shorthands and notations ----------------
%========================================================================================

%====================== double script fonts  =====================================

\global\long\def\RR{\mathbb{R}}
\global\long\def\CC{\mathbb{C}}
\global\long\def\NN{\mathbb{N}}
\global\long\def\QQ{\mathbb{Q}}
\global\long\def\ZZ{\mathbb{Z}}
\global\long\def\EE{\mathbb{E}}
\global\long\def\PP{\mathbb{P}}
\global\long\def\FF{\mathbb{F}}
\global\long\def\11{\mathbbm{1}}

%====================== math bold fonts  =====================================

\newcommand{\bfb}{\mathbf{b}}
\newcommand{\bft}{\mathbf{t}}
\newcommand{\bfs}{\mathbf{s}}
\newcommand{\bfu}{\mathbf{u}}
\newcommand{\bfv}{\mathbf{v}}
\newcommand{\bfw}{\mathbf{w}}

\newcommand{\bfB}{\mathbf{B}}
\newcommand{\bfT}{\mathbf{T}}
\newcommand{\bfU}{\mathbf{U}}
\newcommand{\bfV}{\mathbf{V}}

\newcommand{\bfx}{\mathbf{x}}
\newcommand{\bfX}{\mathbf{X}}
\newcommand{\bfy}{\mathbf{y}}
\newcommand{\bfY}{\mathbf{Y}}
\newcommand{\bfz}{\mathbf{Z}}
\newcommand{\bfZ}{\mathbf{Z}}


%============= Mathcal=============
\def\CalA{\mathcal{A}}
\def\CalB{\mathcal{B}}
\def\CalC{\mathcal{C}}
\def\CalD{\mathcal{D}}
\def\CalH{\mathcal{H}}
\def\CalJ{\mathcal{J}}
\def\CalN{\mathcal{N}}
\def\CalM{\mathcal{M}}
\def\CalP{\mathcal{P}}
\def\CalQ{\mathcal{Q}}
\def\CalR{\mathcal{R}}
\def\CalW{\mathcal{W}}
\def\CalU{\mathcal{U}}
\def\CalV{\mathcal{V}}
\def\CalT{\mathcal{T}}
\def\CalX{\mathcal{X}}
\def\CalY{\mathcal{Y}}

\newcommand{\Cal}[1]{\mathcal{#1}}

%====================== shortcuts for operators  =====================================

\global\long\def\+{\oplus}
\global\long\def\P{\mathsf{P}}

%\newcommand{\prob}{\mathbb{P}}
%\def\<{\langle}
%\def\>{\rangle}

%\newcommand{\sign}{\mathsf{sign}}
%\newcommand{\OR}{\mathsf{OR}}
%\newcommand{\AND}{\mathsf{AND}}
%\newcommand{\MAJ}{\mathsf{MAJ}}

%\newcommand{\abs}[1]{\lvert#1\rvert}
%\newcommand{\norm}[1]{\lVert#1\rVert}
\newcommand{\expec}{\mathbb{E}}

\DeclareMathOperator*{\medcap}{\mathbin{\scalebox{1}{\ensuremath{\bigcap}}}}
\DeclareMathOperator*{\medcup}{\mathbin{\scalebox{1}{\ensuremath{\bigcup}}}}
%\newcommand*{\medcap}{\mathbin{\scalebox{1}{\ensuremath{\bigcap}}}}%
%\newcommand*{\medcup}{\mathbin{\scalebox{1}{\ensuremath{\bigcup}}}}%

\DeclareMathOperator*{\argmin}{arg\,min}
\DeclareMathOperator*{\argmax}{arg\,max}

%-------- delta = for definition -----
\usepackage{stackengine}
\def\deq{\mathrel{\ensurestackMath{\stackon[1pt]{=}{\scriptstyle\Delta}}}}

%===============================================================================
%------------------------- Special Notations -----------------------------------
%===============================================================================

\newcommand{\BigO}[1]{\ensuremath{\operatorname{O}\bigl(#1\bigr)}}
\global\long\def\tensor{\otimes}
%\DeclareMathOperator{\tr}{tr}
 \def\tr{\Tr}
 \def\id{\text{id}}
\global\long\def\bigtensor{\bigotimes}
\allowdisplaybreaks% makes automatic splits of equations

\def\rhon{\rho_{AB}^{\tensor n}}
\def\phirho{\Psi_{RAB}^{\rho_{AB}}}
\def\phirhon{\Psi_{R^nA^nB^n}^{\rho_{AB}}}
\def\distchann{\tilde{\mathcal{N}}}
\def\cdec{\mathsf{P}^{(\mu)}}
\def\TDeltaN{\mathcal{T}_{\delta}^{(n)}}
\def\TDelta{\mathcal{T}_{\delta}}

\def\PiA{\Pi_{\rho^A}}
\def\PiB{\Pi_{\rho^B}}
\def\PihatA{\hat{\Pi}^A}
\def\PihatB{\hat{\Pi}^B}
\def\PiuA{\Pi_{u^n}^A}
\def\PivB{\Pi_{v^n}^B}
\def\PiwA{\Pi_{w^n}}
\def\lambdauA{\lambda^A_{u^n}}
\def\lambdalA{\lambda^A_{l}}
\def\lambdavB{\lambda^B_{v^n}}
\def\lambdakB{\lambda^B_{k}}
\def\lambdawA{\lambda_{w^n}}
\def\lambdaAB{\lambda^{AB}_{u^n,v^n}}
\def\lambdalkAB{\lambda^{AB}_{l,k}}
\def\rhohatuA{\hat{\rho}^A_{u^n}}
\def\rhohatvB{\hat{\rho}^B_{v^n}}
\def\rhohatlA{\hat{\rho}^A_{l}}
\def\rhohatkB{\hat{\rho}^B_{k}}
\def\rhohatwA{\hat{\rho}_{w^n}}
\def\rhohatuAvB{\hat{\rho}^{AB}_{u^n,v^n}}
\def\LambdauA{\Lambda^A_{u^n}}
\def\LambdalA{{\Lambda_l^A}}
\def\LambdavB{\Lambda^B_{v^n}}
\def\LambdakB{\Lambda^B_{k}}
\def\LambdauMuX{\Lambda^{X(\mu)}_{u}}
\def\GammavMuY{\Gamma^{Y}_{v}}
\def\LambdauhatMuX{{\hat{\Lambda}}^{X(\mu)}_{u}}
\def\kappaLKMu{\kappa_{l,k}^{(\mu)}(u^n, v^n)}
\def\TDeltan{\mathcal{T}_{\delta}^{(n)}}
\def\IndiU1{\mathbbm{1}_{\left\{U^{n,(\mu_1)}(l)=u^n\right\}} }
\def\IndiV1{\mathbbm{1}_{\left\{V^{n,(\mu_2)}(k)=v^n\right\}} }
\def\TDeltaN{\mathcal{T}_{\delta}^{(n)}}



%===============================================================================
%------------------------- Special Notations Nov 5th----------------------------
%===============================================================================

\def\sigTilde{\tilde{\sigma}_x}
\newcommand{\eleInSet}[2]{#1\in \mathcal{#2}}
\newcommand{\zeroWithDelta}[1]{#1(\delta) \searrow 0 \text{ as } \delta \searrow 0}
\def\UCodeword{U^{n,(\mu_1)}(a_1,i)}
\def\VCodeword{V^{n,(\mu_2)}(a_2,j)}
\def\WCodeword{W^{n,(\mu)}(a,i)}
\def\WCodewordm{W^{n,(\mu)}(a,m)}
\def\CutOffA{\Pi_A^{\mu_1}}
\def\CutOffB{\Pi_B^{\mu_2}}
\def\CutOff{\Pi^{\mu}}
\def\gammaCoeff{\gamma_{u^n}^{(\mu_1)}}
\def\gammaWCoeff{\gamma_{w^n}^{(\mu)}}
\def\zetaCoeff{\zeta_{v^n}^{(\mu_2)}}
\def\rhotilduA{\tilde{\rho}_{u^n}^A}
\def\rhotildvB{\tilde{\rho}_{v^n}^B}
\def\rhotildlA{\tilde{\rho}_{l}^A}
\def\rhotildkB{\tilde{\rho}_{k}^B}
\def\rhotilduAprime{\tilde{\rho}_{u^n}^{A'}}
\def\rhotildvBprime{\tilde{\rho}_{v^n}^{B'}}
\def\rhotildwA{\tilde{\rho}_{w^n}}
\def\PiTauWn{\Pi_{w^n}^{\theta}}
\def\PiRho{\Pi_{\rho}}
\def\LambdaTildew{\tilde{\lambda}_{w^n}}
\def\IndicSubPOMV{\11_{\{sP\}}}

%% new definitions from purification paper %%%%%%
\def\sigmahatAu{\ket{\hat\sigma_{u^n}}^{AE}}
\def\sigmatildAu{\ket{\tilde\sigma_{u^n}}^{AE}}
\def\sigmahatBv{\ket{\hat\sigma_{v^n}}^{BF}}
\def\sigmatildBv{\ket{\tilde\sigma_{v^n}}^{BF}}
\def\sigmahatAl{{\hat\sigma_{l}}^{AE}}
\def\sigmatildAl{{\tilde\sigma_{l}}^{AE}}
\def\sigmahatBk{{\hat\sigma_{k}}^{BF}}
\def\sigmatildBk{{\tilde\sigma_{k}}^{BF}}
\def\PsiRhoN{\Psi_{\rho^{\tensor n}}^{ABCR}}
\def\PsiRhoNket{\ket{\Psi_{\rho^{\tensor n}}}^{ABCR}}
\def\clocc{$1$\mbox{-CLOCC}^\prime}
\newcommand{\ral}{\rangle}
\newcommand{\lal}{\langle}
% \newcommand{\settildeR}[2]{#1 \in [1,2^{n\tilde{R}_{#2}}]}

\newcommand{\settildeR}[2]{#1 \in [2^{n\tilde{R}_{#2}}]}
\newcommand{\Unitary}[2]{U_{\scriptscriptstyle \!#1}^#2}

%% ----------- coloring defs ----------------------------------
\newcommand{\checkComm}[1]{\textcolor{blue}{#1}}
\newcommand{\error}[1]{\textcolor{red}{#1}}

